A Kepler's note on secular inequalities

I discuss the problem of secular inequalities in Kepler by giving account of a manuscript note that has not been published until 1860. In his note Kepler points out the need for a model, clearly inspired by the method of epicycles, that describes the secular inequalities as periodic ones. I bring attention to this point, that seems to have been underestimated, since the references to Kepler's work usually report only that he observed a decreasing mean motion for Saturn and an increasing one for Jupiter.

==> tab_simboli.tex <==
\table{oss.simboli}{I simboli usati in astronomia per identificare i
pianeti ed i segni dello zodiaco.}{\vbox{\tabskip=0pt\offinterlineskip
\parindent 0pt\tabskip 0pt\halign{
\vrule$\phantom{\Big\vert}$\hfil
{\quad}{#}
&{\ }{#}\hfil{\quad}\vrule
&{\quad}{#}
&{\ }{#}\hfil{\quad}\vrule
&{\quad}{#}
&{\ }{#}\hfil{\quad}\vrule
\cr
\noalign{\hrule}
\astrosun & Sole      & \rightmoon & Luna     &           &         \cr
\mercury  & Mercurio  & \venus    & Venere   & \earth    & Terra   \cr
\mars     & Marte     & \jupiter  & Giove    & \saturn   & Saturno \cr
\uranus   & Urano     & \neptune  & Nettuno  & \pluto    & Plutone \cr
\noalign{\hrule}
\aries       & Ariete     & \taurus   & Toro      & \gemini      & Gemelli    \cr
\cancer      & Cancro     & \leo      & Leone     & \virgo       & Vergine    \cr
\libra       & Bilancia   & \scorpio  & Scorpione & \sagittarius & Sagittario \cr
\capricornus & Capricorno & \aquarius & Acquario  & \pisces      & Pesci      \cr
\noalign{\hrule}
}}}

